Cross-Layer Optimization for Power-Efficient and Robust Digital Circuits and Systems

With the increasing digital services demand, performance and power-efficiency become vital requirements for digital circuits and systems. However, the enabling CMOS technology scaling has been facing significant challenges of device uncertainties, such as process, voltage, and temperature variations. To ensure system reliability, worst-case corner assumptions are usually made in each design level. However, the over-pessimistic worst-case margin leads to unnecessary power waste and performance loss as high as 2.2x. Since optimizations are traditionally confined to each specific level, those safe margins can hardly be properly exploited. To tackle the challenge, it is therefore advised in this Ph.D. thesis to perform a cross-layer optimization for digital signal processing circuits and systems, to achieve a global balance of power consumption and output quality. To conclude, the traditional over-pessimistic worst-case approach leads to huge power waste. In contrast, the adaptive voltage scaling approach saves power (25% for the CORDIC application) by providing a just-needed supply voltage. The power saving is maximized (46% for CORDIC) when a more aggressive voltage over-scaling scheme is applied. These sparsely occurred circuit errors produced by aggressive voltage over-scaling are mitigated by higher level error resilient designs. For functions like FFT and CORDIC, smart error mitigation schemes were proposed to enhance reliability (soft-errors and timing-errors, respectively). Applications like Massive MIMO systems are robust against lower level errors, thanks to the intrinsically redundant antennas. This property makes it applicable to embrace digital hardware that trades quality for power savings.

==> abstract.tex <==
\chapter{Abstract}\label{ch:abstract}
With the increasing digital services demand, performance and power-efficiency become vital requirements for digital circuits and systems. However, the enabling CMOS technology scaling has been facing significant challenges of device uncertainties, such as process, voltage, and temperature variations. To ensure system reliability, worst-case corner assumptions are usually made in each design level. However, the over-pessimistic worst-case margin leads to unnecessary power waste and performance loss as high as 2.2x. Since optimizations are traditionally confined to each specific level, those safe margins can hardly be properly exploited.

To tackle the challenge, it is therefore advised in this Ph.D. thesis to perform a cross-layer optimization for digital signal processing circuits and systems, to achieve a global balance of power consumption and output quality.


The first key contribution of this work is an algorithm to identify important flip-flops that contribute significantly to circuit outputs, by analytically modeling reliability threats at logic gate-level. Consequently, circuit designers are guided on which flip-flop to harden against random errors (on ASIC, e.g. FFT, LDPC decoder). With this help, this thesis eliminated the unnecessary hardening overheads (achieving the same SNR with only half of hardening overheads) for a traditional FFT design.
This work also contributes by optimizing the micro-architecture for the embedded OpenRISC processor, exploiting application-level word-length opportunities. It improved the power efficiency for universal signal processing applications. For instance, It saved power by 9.5\% for the whole execution unit on the Coremark benchmark.
Moreover, this work mitigated circuit-level errors in micro-architectural and algorithm levels for recursive applications. The techniques were applied on a CORDIC hardware accelerator in digital front-end, which saves power consumption by up to 46\%.
The last key contribution of this thesis is the algorithm and application-level optimization to mitigate lower-level errors on Massive MIMO wireless communication systems. It demonstrated that for typical Massive MIMO setup, a few (3\%) antenna outage will only degrade the target system SNR by 0.5dB. This promotes operating the circuit in a more aggressive region, which might lead to circuit errors, to improve power efficiency.

To conclude, the traditional over-pessimistic worst-case approach leads to huge power waste. In contrast, the adaptive voltage scaling approach saves power (25\% for the CORDIC application) by providing a just-needed supply voltage. The power saving is maximized (46\% for CORDIC) when a more aggressive voltage over-scaling scheme is applied. These sparsely occurred circuit errors produced by aggressive voltage over-scaling are mitigated by higher level error resilient designs. For functions like FFT and CORDIC, smart error mitigation schemes were proposed to enhance reliability (soft-errors and timing-errors, respectively). Applications like Massive MIMO systems are robust against lower level errors, thanks to the intrinsically redundant antennas. This property makes it applicable to embrace digital hardware that trades quality for power savings.


%\instructionsabstract


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> abstractnl.tex <==
\chapter{Nederlandstalige Synopsis}

Met de toenemende vraag naar digitale diensten worden prestaties en vermogen-efficiëntie  energie-efficiëntie essentiële vereisten voor digitale circuits en systemen. De schaling van CMOS technologie die dit mogelijk maakt, wordt echter  geconfronteerd met belangrijke uitdagingen door onzekerheden in geminiaturiseerde componenten, zoals proces-, spanning- en temperatuurvariaties. Om de betrouwbaarheid van systemen te waarborgen, worden meestal in alle ontwerpniveaus conservatieve marges voorzien. Deze aannames zijn echter te pessimistisch, en de genomen marges zorgen voor energieverspilling en prestatieverlies dat kan oplopen tot een factor 2.2 van wat haalbaar is door de technologie. Aangezien de  optimalisaties traditioneel beperkt zijn tot elk specifiek niveau, kunnen deze veilige marges niet goed worden benut.

Om deze uitdaging aan te pakken, wordt het daarom geadviseerd in dit Ph.D. proefschrift om een cross-layer optimalisatie uit te voeren voor digitale signaalverwerkingscircuits en systemen, om een globaal evenwicht te bereiken tussen stroomverbruik en kwaliteit aan de uitgangen van de schakelingen.

De eerste sleutelbijdrage van dit werk is een algoritme om belangrijke flip-flops te identificeren die aanzienlijk bijdragen aan de uitgangen van het circuit, door analytische modellering vanbetrouwbaarheidsdrempels op logisch poortniveau. Bijgevolg worden circuitontwerpers begeleid om enkel een hogere marge te nemen op flip-flops die gevoeliger zijn voor willekeurige fouten (bijvoorbeeld FFT, LDPC decoder circuits in een applicatie specifieke schakeling). Met deze hulp elimineerde dit proefschrift de onnodige marges op de helft van de flipflopseen traditioneel FFT-ontwerp, en kon een identieke kwaliteit bekomen worden als het conservatief ontwerp.
Dit werk draagt ook bij aan het optimaliseren van de micro-architectuur van een microprocessor voor het verbeteren van de energie-efficiëntie voor universele signaalverwerking toepassingen . Dit verbeterde de energie-efficiëntie van de verwerkingseenheid van een OpenRisc processor met 9.5\%  voor de volledige Coremark benchmark .
Bovendien verminderde dit werk fouten op circuitniveau in micro-architecturale en algoritme-niveaus voor recursieve toepassingen. De technieken werden toegepast op een CORDIC hardware accelerator in digitale front-end, waardoor een besparing van energieverbruik met 46\% wordt bekomen.
De laatste belangrijke bijdrage van dit proefschrift is het optimaliseren van de algoritme en applicatie om de fouten van de Massive MIMO draadloze communicatiesystemen te beperken. Het blijkt dat voor een typische Massieve MIMO-installatie antenne-uitval van 3\% de signaal ruis verhoudingslechts met 0.5 dB zal degraderen. Dit laat toe de electronische circuits te laten werken in een foutgevoeliger gebied, om de energie-efficiëntie van het totaal systeem gevoelig te verbeteren.

Tenslotte stelden we vast dat de traditionele keuze voor pessimistische marges inderdaad tot gevoelige vermogentoename leiden. In tegenstelling hiermee bespaart de adaptieve spanningsschaalbenadering energie (25\% voor de CORDIC-toepassing) door de benodigde voedingsspanning te beperken. De energiebesparing wordt gemaximaliseerd (46\% voor CORDIC) wanneer een meer agressieve spanningsoverschaling wordt toegepast. Deze zelden voorkomende schakelfouten, die worden veroorzaakt door agressieve verlagen van de spanning, worden vermeden door een robuuster ontwerp op hogere niveaus van de meest gevoelige schakelingen. Voor functies zoals FFT en CORDIC werden slimme foutverminderingsschema's voorgesteld om de betrouwbaarheid te verbeteren (respectievelijk softfouten en timingfouten). Toepassingen zoals Massive MIMO-systemen zijn robuust tegen hoger fouten, dankzij de intrinsieke redundante antennes. Deze eigenschap laat to om kwaliteit af te wegen ten opzichte van energiebesparing voor digitale hardware.





%\instructionsabstract

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> curriculum.tex <==
\chapter{Curriculum Vitea}\label{ch:curriculum}

Yanxiang Huang received the B.Sc. degree in 2011 from Zhejiang University, China, and the M.Sc. degree in 2013 from Eindhoven Technology University (TU/e), the Netherlands, both in electrical engineering. Since November 2013, he has been working toward the Ph.D. degree in the Department of Electrical Engineering (ESAT) at University of Leuven (KU Leuven), with his research activities performed in collaboration with imec, Leuven, Belgium.

During 2012 to 2013, he served as a research intern in Research Division, NXP semiconductors, Eindhoven, the Netherlands. Since 2013, he has been working as a Ph.D. researcher in the Perceptive System Group, imec, Leuven, Belgium.

His research interest includes the design of digital circuits and systems, digital hardware units for wireless communication, IoT devices, multimedia accelerators, low-power computing, reliability, and algorithm-architecture co-exploration for digital computing.


%\instructionscv


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> preface.tex <==
\chapter{Acknowledgements} \label{sec:preface}

Undertaking this Ph.D. has been a truly life-changing experience for me. It would not have been possible without the support and guidance that I received from many people. It is a pleasure for me to take this opportunity to express my gratitude.


First of all, I would like to express my deep and sincere appreciation to my supervisors, Prof. Wim Dehaene and Prof. Liesbet Van der Perre. I have been incredibly lucky to have both as my advisors. Prof. Liesbet Van der Perre offered me the opportunity, backed in 2013 autumn, to pursue this research subject that I passionate. She always keeps faith in my work and provides full support in every aspect of my research, spanning from the knowledge on wireless communication systems, to scientific writing and even career advice. Prof. Wim Dehaene joined as my promoter in 2014 winter. He brings not only world-class understanding of circuits and systems, inspiring consultations on professional and personal developments. Furthermore, I would like to thank my committee member Prof. Francky Catthoor, for providing critical comments on my work, and for teaching me the enthusiastic attitude towards research. My cordial gratefulness also goes to all the jury members: Prof. Sofie Pollin, Prof. Rudy Lauwereins, Prof. Andreas P. Burg, and Prof. Liang Liu. It is their feedback that significantly improves this work.



My sincere thank goes to Andre Bourdoux, for his scientific supervision from the imec perceptive. I would like to thank Chunshu Li, towards whom I can share all the ideas freely. His advice helps shape a lot of the flashing thoughts towards research ideas. I would also express my appreciation to Meng Li. She has always been very supportive since the first day I joined imec.


Besides, I would like to express my gratitude my superb colleagues from the perceptive system group in imec, Maxim Rykunov, Khaled Khalaf, Claude Desset, Veerle Derudder, Qixian Shi, Hans Cappelle, Hans Suys, Simone Corbetta, Eddy De Greef, Miguel Glassee, and Karthick Parashar. Thank you for your warm help when I came to you with mathematics formulation, Matlab code, system description, circuit simulation or even Latex code.
Moreover, I would like to thank the group management and administration, Wim Van Thillo, Andy Dewilde, Charlotte Soens, Annemie Stas, and Bjorn Debaillie, for their supportive assistance with the practical issues during the past years, especially scheduling tape-outs, conferences attendance, and measurement equipment.


Furthermore, I would like to thank various colleagues from imec, Peter Debacker, Min Li, Julien Verschueren, Sebastien Morrison, Paul Zuber, Petr Dobrovolny, Phillip Christie, Steven Redant, for the enjoyable cross-discipline collaborations. I am also very grateful for the colleagues from the KU Leuven, Chunming Liu, and Andras Boho for the inspiring discussions. 

I am deeply grateful to my Ph.D. friends, Halil Kukner, Matthias Hartmann, Prashant Agrawal, Ubaid Ahmad, Steve Blandino, Alessandro Chiumento, Raf Appeltans, Oscar Elisio Mattia, Johan Nguyen, for the special `Ph.D.' moments. My warm gratitude also goes to Zhijie Xu, Habib Khalid, Yuzhu Gai, Antonio Callejon, Sara Gunnarsson, and Miceale Bortas, for the splendid cooperation during their master thesis. 


Moreover, I would like to share my gratitude towards the friends from imec and KU Leuven, Michael Chen, 
Xiaoqiang Zhang, Zhiwei Zong, Yao Liu, Cheng-Hsueh Tsai,
Leqi Zhang, Linkun Wu, Mingxu Liu, Weiming Qiu, Tiwei Wei, Menglei Xu, Chang Chen, Ziyang Liu, Dongjie Shao, Gaozhan Cai, Xin Lin, Jiachen Wang, Xueji Zhang, many others and their family members, for invaluable help and consultant in all aspects.


Finally, I especially owe my loving thanks to my family. The trust and encouragement from my parents helped me to overcome every difficulty and will motivate me achieving any other success in the future. I devote my deepest gratitude to my wife, Dan Ning. We met, got acquaintance, and finally got married during my Ph.D. study in Leuven. This thesis would not have been possible without her warming hug, understanding, encouragement, and most importantly, love.


\begin{flushright}
Yanxiang Huang

September 2017

Leuven, Belgium
\end{flushright}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Keep the following \cleardoublepage at the end of this file, 
% otherwise \includeonly includes empty pages.
\cleardoublepage

% vim: tw=70 nocindent expandtab foldmethod=marker foldmarker={{{}{,}{}}}


==> publications.tex <==
\chapter{List of publications}\label{sec:pub}



%%%%%%%%%%%%
%% Journal
%%%%%%%%%%%%
\begin{refsection}
\nocite{huang16jsps-error-resilient}
\nocite{huang16el-hardware-switch}
\nocite{li16jsps-polar-dfe}
\nocite{li15el-ldpc}
\nocite{huang15micpro-deci-filter}

\newrefcontext[sorting=none]
\printbibliography[title={Journal (Authored and Co-Authored)},heading=subbibliography, env=midbib]
\end{refsection}




%%%%%%%%%%%%
%% patent
%%%%%%%%%%%%
\begin{refsection}

\nocite{huang16us-error-resilient}
\nocite{li15us-polar-dfe}

\newrefcontext[sorting=none]
\printbibliography[title={Patents (Authored and Co-Authored)},heading=subbibliography, env=midbib]
\end{refsection}


%%%%%%%%%%%%
%% conference
%%%%%%%%%%%%
\begin{refsection}
\nocite{huang17icassp-mimo-dfe}
\nocite{gunnarsson17eucnc-loussy-processing}
\nocite{huang16dac-serial}
\nocite{huang16asscc-polar-dfe}
\nocite{huang15wapco-error-resilient}
\nocite{li15icassp-polar-dfe}
\nocite{li15asscc-ldpc}
\nocite{huang14sips-error-resilient}
\nocite{callejon14wic-turbo}
\nocite{huang13norchip-deci-filter}


\newrefcontext[sorting=none]
\printbibliography[title={Conferences and Workshops (Authored and Co-Authored)},heading=subbibliography, env=midbib]
\end{refsection}





%%%%%%%%%%%%
%% reports
%%%%%%%%%%%%
\begin{refsection}


\nocite{huang13thesis-deci-filter}

\newrefcontext[sorting=none]
\printbibliography[title={Reports},heading=subbibliography, env=midbib]
\end{refsection}






%%%%%%%%%%%%
%% WIP
%%%%%%%%%%%%
%\begin{refsection}

%\nocite{}

%\printbibliography[title={Papers in progress (Authored and Co-Authored),heading=subbibliography]
%\end{refsection}






%\sloppy
%
%\cvsubsection{Journals}
%\printbibliography[heading=none, type = article ]
%
%\cvsubsection{Patents}
%\printbibliography[heading=none, type = misc ]
%
%\cvsubsection{Conferences}
%\printbibliography[heading=none, type = inproceedings] % title = conference
%
%\cvsubsection{Thesis}
%\printbibliography[heading=none, nottype = article,  nottype = misc, nottype = inproceedings]
%%\printbibliography

